FedPM: Federated Learning Using Second-order Optimization with Preconditioned Mixing of Local Parameters

We propose Federated Preconditioned Mixing (FedPM), a novel Federated Learning (FL) method that leverages second-order optimization. Prior methods--such as LocalNewton, LTDA, and FedSophia--have incorporated second-order optimization in FL by performing iterative local updates on clients and applying simple mixing of local parameters on the server. However, these methods often suffer from drift in local preconditioners, which significantly disrupts the convergence of parameter training, particularly in heterogeneous data settings. To overcome this issue, we refine the update rules by decomposing the ideal second-order update--computed using globally preconditioned global gradients--into parameter mixing on the server and local parameter updates on clients. As a result, our FedPM introduces preconditioned mixing of local parameters on the server, effectively mitigating drift in local preconditioners. We provide a theoretical convergence analysis demonstrating a superlinear rate for strongly convex objectives in scenarios involving a single local update. To demonstrate the practical benefits of FedPM, we conducted extensive experiments. The results showed significant improvements with FedPM in the test accuracy compared to conventional methods incorporating simple mixing, fully leveraging the potential of second-order optimization.

==> sec5_limitations.tex <==
\section{Limitations and future work}

\noindent
\textbf{Limitations in convergence analysis}: The current theoretical analysis of FedPM presented in Sec. \ref{subsec:analysis} is restricted to scenarios involving a single local update $(K=1)$ per communication round. While this provides a solid foundation, extending the analysis involving multiple local updates remains an open challenge. Such an extension is crucial for evaluating the robustness and efficiency of FedPM in practical settings, where multiple local updates are typically employed to reduce communication overhead. Furthermore, our analysis focuses on strongly convex models; extending it to non-convex models introduces additional challenges. 

\noindent
\textbf{Unexplored theoretical analysis of preconditioner approximations}: In Sec. \ref{subsec:approx}, we outlined a practical preconditioner approximation (FOOF). However, the theoretical implications of this approximation, particularly their impact on convergence rates, have not been analyzed. Addressing this gap would enhance the theoretical guarantees and provide deeper insights into its efficacy.

\noindent
\textbf{Communication efficiency}: Although FedPM mitigates some communication inefficiencies inherent in second-order optimization, the additional transmission of preconditioners introduces communication overhead. Exploring strategies to further optimize communication without preserving convergence performance is a valuable direction for future work.


